Leveraging Model-based Trees as Interpretable Surrogate Models for Model Distillation

Surrogate models play a crucial role in retrospectively interpreting complex and powerful black box machine learning models via model distillation. This paper focuses on using model-based trees as surrogate models which partition the feature space into interpretable regions via decision rules. Within each region, interpretable models based on additive main effects are used to approximate the behavior of the black box model, striking for an optimal balance between interpretability and performance. Four model-based tree algorithms, namely SLIM, GUIDE, MOB, and CTree, are compared regarding their ability to generate such surrogate models. We investigate fidelity, interpretability, stability, and the algorithms' capability to capture interaction effects through appropriate splits. Based on our comprehensive analyses, we finally provide an overview of user-specific recommendations.

==> chapters/4_Selection_Bias.tex <==
\subsection{Definition and motivation}

According to \cite{Hothorn.2006} an algorithm for recursive partitioning is called unbiased when, under the conditions of the null hypothesis of independence between a response $y$ and feature $\textbf{x}_{1},...\textbf{x}_{p}$ the probability of selecting feature $\textbf{x}_{j}$ is $1/p$ for all $j = 1,...,p$ regardless of the measurement scales or the number of missing values.

This definition may be surprising at first, since if there is no dependency between the target and the features, one would not want to perform a split anyway and would try to prevent this through appropriate pruning procedures.
However, the idea behind this is that if, in the case of independence, a feature with, for example, a large number of possible split points is selected more frequently as a splitting feature than a feature with a smaller number of split points, the former could also be incorrectly selected more frequently as a splitting feature if there is a dependency on the response for the second feature.
\cite{Loh.2014}

In the discussion on the Paper Fifty Years of Classification and Regression Trees of \cite{Loh.2014}, Carolin Strobl's statement on selection bias is therefore very clear:
\vspace{0.5cm}


{\par\centering \textit{"One should think that the results shown here [...] are so clear that any statistically educated person should never
want to use a biased recursive partitioning algorithm again."}\par}
\vspace{0.5cm}

So if SLIM is the only biased algorithm, it would have to be discarded immediately according to this statement. However, this will be investigated in detail in the following.



\subsection{Simulation independence scenarios}
In order to empirically investigate whether the four algorithms presented actually correspond to the respective groups (biased and unbiased) using the definition of \cite{Hothorn.2006}, two different simulations were carried out.

In the first scenario, only numerical features are used, whereas in the second scenario numerical features and additionally one binary and two categorical features are considered.

\paragraph{Independence numeric\\}
The data in the first scenario is defined as follows:
\begin{itemize}
    \item $\textbf{x}_{1}, \textbf{x}_{2} \sim U(0,1)$
    \item $\textbf{x}_3$ uniformly distributed on the set $\{0, 0.1,..., 0.9, 1\}$
    \item $\textbf{x}_4$ uniformly distributed on the set $\{0, 0.01,..., 0.99, 1\}$
    \item $y \sim N(0,1)$
    \item sample size $n = 1000$
    \item 1000 simulation runs
\end{itemize}

The resulting frequencies are shown in Figure \ref{fig:selection_bias_independence_numeric} and are consistent with the expectations. SLIM clearly prefers to select features with a higher number of split points and therefore is biased. The other three methods seem to  select all four features about the same number of times.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=10cm]{figures/independence_numerical.png}
    \caption{Simulated frequencies of selected splitting features for scenario independence numeric}   \label{fig:selection_bias_independence_numeric}
\end{figure}



\paragraph{Selection bias independence mixed \newline}
In the second scenario, the data is simulated as follows:
\begin{itemize}
    \item $\textbf{x}_{1}, \textbf{x}_{2} \sim U(0,1)$
    \item $\textbf{x}_3$ uniformly distributed on the set $\{0, 0.1,..., 0.9, 1\}$
    \item $\textbf{x}_4  \sim Bern(0.5)$
    \item $\textbf{x}_5$ uniformly distributed on 5-factor levels (15 possible splits)
    \item $\textbf{x}_6$ uniformly distributed on 8-factor levels (128 possible splits) %stirling number of second kind
    \item $y \sim N(0,1)$
    \item sample size $n = 1000$
    \item 1000 simulation runs
\end{itemize}

The addition of categorical features in this scenario results in a different picture for the frequencies, as shown in Figure \ref{fig:selection_bias_independence_mixed}. Although the numerical features are chosen with approximately equal frequency in the so-called "unbiased" methods, there are large deviations in the binary and categorical features especially for MOB and CTree, which calls the designation "unbiased" into question.
A possible explanation for this selection bias could be that due to the large number of parameters that have to be estimated for the categorical features in the modeling step, random dependencies to the target variable are already caught well in the model  and therefore these features are used less frequently as splitting features.


In \cite{Hothorn.2006} the unbiasedness of CTree is empirically investigated for cases, in which a strict separation between regressor features and partitioning features is kept. Therefore, the result shown here should not principally question the label, but it does not seem appropriate when there is an overlap or, as in our case, even congruence between the two roles.


\begin{figure}[!htb]
    \centering
    \includegraphics[width=14cm]{figures/independence_mixed.png}
    \caption{Simulated frequencies of selected splitting features for scenario independence mixed}
    \label{fig:selection_bias_independence_mixed}
\end{figure}

For GUIDE two different variants were evaluated in this scenario. "GUIDE excl cat" corresponds to the original version, in which categorical features are only used as splitting and not as regressor features. In "GUIDE incl cat", on the other hand, the categorical features are also used as regressors. The fact that the frequencies of the categorical features are smaller in "GUIDE incl. cat" could be explained analogously to the selection bias of MOB and CTree.

The binary feature $\textbf{x}_4$ is almost never chosen as a splitting feature with SLIM, in contrast to the other features. However, this can be attributed to the selection bias in numerical features with different numbers of split points, as the binary feature can be seen as a numerical feature with only one possible split point. What is more interesting is that the numerical feature $\textbf{x}_2$ with 10 possible split points is chosen by SLIM much more frequently as a splitting feature than the feature $\textbf{x}_6$ with 128 possible splits, so that the bias cannot be determined by the number of possible splits alone.

The difference between the categorical ($\textbf{x}_5$ and $\textbf{x}_6$) and the numerical features can probably be explained in a similar way as with the other methods but in reverse. With SLIM, the potential split is executed first and then models in the child nodes are fitted.  If a numerical feature is used as a partitioning feature, the parameters for all factor levels are estimated in both child models, whereby random dependencies with $y$ can be modeled very accurately. If, on the other hand, splitting is done according to a categorical feature, only a subset of the factor levels can be used for modeling in both child nodes.






As a possible correction approach for the selection bias in SLIM, I investigated how the number of quantiles considered as potential split points affects the selection bias and the performance of SLIM. The simulation setup and results are shown in the Online~Appendix~\ref*{app:selection_bias_correction}~\cite{HLDEC23}. In summary, although selection bias can be reduced for numerical features in the case of an independent target variable, this correction can lead to unpredictable biases if interactions are actually present. For this reason, the approach is not recommended.
For all simulations in this chapter, each unique value was seen as a potential split point for SLIM.






\subsection{Simulation interaction scenarios} \label{selection_bias_interactions}
While so far only the frequencies with which different feature types are selected in the case of independence were shown, it is empirically investigated in the following which feature types the different MBT algorithms tend to select when interactions are actually present.
Four different scenarios are examined for this. These are, in a sense, pair comparisons of different feature types. In all scenarios, the data generating process consists of two pairs of interactions, whereby the interactions have the same strength. Each pair consists of a numerical feature that enters linearly into the interaction and another feature that splits the linear effect into two subgroups.
In all four scenarios, the numerical features which define the linear effect are
 $\textbf{x}_{2}, \textbf{x}_{4} \sim U(0,1)$ .

The features $\textbf{x}_{1}$ and $\textbf{x}_{3}$ are responsible for the subgroups. They are uniformly distributed on sets, which are given in Table \ref{tab:selection_bias_interaction}, as well as the data generating processes.

\begin{table}[!htb]
    \centering
    \begin{tabular}{llll}
        \hline
        scenario & $\textbf{x}_1$ & $\textbf{x}_3$ & $f(\textbf{x})$\\
        \hline
        numerical vs numerical & $[0,1]$ &  $\{0, 0.1,..., 0.9, 1\}$ & $\mathbb{1}_{(\textbf{x}_1 \leq  mean(\textbf{x}_1))}\textbf{x}_2  +  \mathbb{1}_{(\textbf{x}_3 \leq  mean(\textbf{x}_3))}\textbf{x}_4 $ \\
        binary vs categorical & $\{0,1\}$ &  $\{a,b,c,d,e,f\}$ & $\mathbb{1}_{(\textbf{x}_1 = 0)}\textbf{x}_2  +  \mathbb{1}_{(\textbf{x}_3 \in \{a,b,c\})}\textbf{x}_4 $ \\
        numerical vs binary & $[0,1]$ & $\{0,1\}$ & $\mathbb{1}_{(\textbf{x}_1 \leq  mean(\textbf{x}_1))}\textbf{x}_2  +  \mathbb{1}_{(\textbf{x}_3 = 0)}\textbf{x}_4$ \\
        numerical vs categorical & $[0,1]$ & $\{a,b,c,d,e,f\}$ & $\mathbb{1}_{(\textbf{x}_1 \leq  mean(\textbf{x}_1))}\textbf{x}_2  +  \mathbb{1}_{(\textbf{x}_3 \in \{a,b,c\})}\textbf{x}_4$ \\
        \hline
    \end{tabular}
    \caption{Simulation scenarios selection bias interaction}
    \label{tab:selection_bias_interaction}
\end{table}





All experiments are repeated 1000 times. The error terms are set to $\epsilon \sim N(0, 0.1 \cdot sd(f(\textbf{x}))$ and the data generating processes are $y = f(\textbf{x}) + \epsilon$.



First of all, there is the question of how selection bias should be defined in these scenarios. Transferring the definition from the independence case, one possibility would be to require that the frequency of being selected as a split feature for all features is 1/4.  However, this does not take into account that splits according to $\textbf{x}_1$ and $\textbf{x}_3$, i.e. according to the split features that define the subgroups, produce a considerably greater improvement in performance than splits according to the smooth features $\textbf{x}_2$  and $\textbf{x}_4$. If $\textbf{x}_1$  and $\textbf{x}_3$  are chosen preferentially, one should not regard this as selection bias but as a good splitting strategy to get the smallest and best-performing trees possible. What could be expected from an unbiased procedure, however, is that both interaction pairs are chosen equally often for the first split.



\begin{figure}[!htb]
    \centering
    \includegraphics[width = 16cm]{figures/interactions.png}
    \caption{Simulated frequencies of selected splitting features for the four interaction scenarios}
    \label{fig:selection_bias_interactions}
\end{figure}

Figure \ref{fig:selection_bias_interactions} shows the frequencies of the first selected split feature in each scenario for each MBT. It can be seen that in none of the scenarios and for none of the MBTs the results seem to be equally distributed among all four features.
As a general rule, it is noticeable that SLIM and GUIDE always prefer the subgroup-defining features ($\textbf{x}_1$  and $\textbf{x}_3$) for splitting, while CTree always prefers the smooth features. For MOB, the behavior varies depending on the feature type.

In Scenario "numerical vs numerical", the distribution for MOB and CTree is at least evenly distributed between the two interaction pairs. One could therefore speak of unbiasedness here. However, while CTree only uses the linear features $\textbf{x}_2$ and $\textbf{x}_4$ as the first split feature, MOB splits according to the subgroup-defining features, which is preferable in practice.
In GUIDE and SLIM, only the features $\textbf{x}_1$ and $\textbf{x}_3$ are selected, but there seems to be a preference for the feature $\textbf{x}_1$, which has a larger number of potential split points.


In the scenario "binary vs categorical", the distribution between the two interaction pairs seems to be roughly equal for SLIM, MOB, and CTree. In contrast to the first scenario, MOB does not split according to the subgroup-defining features but with regard to the linear features.
In GUIDE, only the binary feature is selected, so there is a clear preference for the binary feature over the categorical feature.

In the remaining scenarios, a strong selection bias is evident in all MBTs. SLIM, for example, gives considerable preference to numerical subgroup-defining features over binary and categorical features.





Obviously, these scenarios do not represent a complete overview of possible interactions. However, since MBTs can show their strengths, especially in the presence of subgroup-specific main effects (i.e. good interpretability through small trees but good performance at the same time), only such scenarios are compared here. These simulation results should sensitize to the fact that in certain cases features could only be selected as splitting features because they have certain properties and not because their share in an interaction is the largest, even with the so-called unbiased methods.

Finally, it should be noted that even if selection bias is present in the independence case, this does not necessarily lead to the wrong feature being selected for splitting. In particular, this can often be prevented by pruning. However, as far as could be observed here, selection bias is very difficult to control or predict and should therefore always be considered when using these algorithms.





%\textbf{Test for selection bias:} $\chi^2$ goodness of fit test\\
%H0: the probabilities of the population are all equal (or are equal to an assumed probability distribution p)







==> chapters/6_Insurance_use_case.tex <==
In the following, SLIM is used in various configurations as a surrogate for modelling the benefit present values of two fictitious insurance tariffs from the TRAIL.X (TRustworthy Artificial Intelligence in Life Insurance) research project \cite{msginsurit.16.03.2023}. The results are interpreted and the fidelity is compared with the MBT algorithms GUIDE, MOB and CTree.

\subsection{Data set K2204} \label{K2204_BPV}

The data set K2204 contains data for a (fictitious) endowment insurance tariff. With this tariff, a single benefit is paid both in the event of survival and death of the policyholder. The data set includes the features sex (1 = male, 0 = female), age and duration and the two targets benefit present value (BPV) and premium present value (PPV). The targets were modelled using two different black box models.  
In the following, only the BPV is used. The results for the PBV are very similar (interpreted the other way round) and can be found in the appendix.
Since the data set with 5994 observations is rather small, all observations were used for training. For this data set therefore only training performance of the surrogate models is considered.
A special characteristic of K2204 is a correlation between the features age and duration, as can be seen in Figure \ref{fig:ins_corr_age_duration}. When interpreting a MBT for this data set, it must therefore be taken into account that a split with regard to one of the features can have an influence on the value range of the other feature.

\begin{figure}[!htb]
    \centering    
    \includegraphics[width=5cm]{figures/corr_age_duration.png}
    \caption{Features age and duration in the K2204 data set}
    \label{fig:ins_corr_age_duration}
\end{figure}


\subsubsection{Shallow MBTs with linear models}
In a first step, SLIM is fitted as surrogate to the black box predictions of BPV (BPV\_pred) with linear regression models in the nodes. The maximum depth is set to 3 and an improvement in the objective ($impr$) of at least $0.1$ of the previous improvement is set as prepruning parameter.
 The resulting tree is shown in Figure \ref{fig:ins_slim_lm_tree}.

 \begin{figure}[!htb]
     \centering     
     \includegraphics[width = 14cm]{figures/slim_lm_tree.png}
     \caption{SLIM tree for K2204 with linear models}
     \label{fig:ins_slim_lm_tree}
 \end{figure}

Basic observations across all subregions are:
\begin{itemize}
    \item Gender male has a positive effect on BPV\_pred
    \item age has a positive effect on BPV\_pred
    \item duration has a negative effect on BPV\_pred
\end{itemize}

The strength of the effects, however, differs in the different subregions found by SLIM.
The five leaf nodes can be roughly divided into two regions with similar effects:
\begin{itemize}
    \item Region 1 (Nodes 2,8): High duration ($30$) or high age ($>48$) and medium duration (between $13$ and $30$)
    \item Region 2 (Nodes 5,6,7): Low - medium duration with low age or high age with low duration ($\leq 12$)
\end{itemize}

In Region 1 sex male and age seem to have a higher positive effect on  BPV\_pred than in region 2. The negative effect of duration, on the other hand, is smaller in region 1. This indicates a nonlinearity of duration.

If SLIM is fitted as a standalone model instead of a surrogate model in the same configuration, the differences in the split points are very small. This indicates that the black box model captures the underlying relationships very well. The corresponding tree is shown in the appendix in Figure \ref{fig:app_ins_slim_lm_standalone_tree}.

In the following, the fidelity of the different MBT with algorithms with linear models is compared. For this purpose, all four algorithms were fitted with a maximum depth of 3. For SLIM and GUIDE, $impr$ is set to $0.05$ and for MOB and CTree $alpha$ is set to $0.05$. Furthermore, a minimum node size of 200 observations is required.
The MBTs are compared with a baseline model, which is a linear regression model on the entire feature space. In addition to the $R^2$ and the MSE, the mean absolute error (MAE) and the maximum absolute error (max AE) are included as measures of fidelity. The max AE is particularly important here, as it is strictly regulated in order not to discriminate against any individual. 
The results are listed in Table \ref{tab:ins_k2204_lm_surrogates_perf}. It shows that all MBTs achieve considerable improvement over the baseline model.

\begin{table}[!htb]

\centering \scriptsize
\begin{tabular}[t]{l|r|r|r|r|r}
\hline
  & $R^2$ & MSE & MAE & max AE & n leaves\\
\hline
linear baseline model & 0.985101 & 0.000201 & 0.011393 & 0.064709 & 1\\
\hline
SLIM & 0.999233 & 0.000010 & 0.002272 & 0.020526 & 8\\
GUIDE & 0.999276 & 0.000010 & 0.002142 & 0.020526 & 8\\
MOB & 0.998527 & 0.000020 & 0.003149 & 0.024504 & 8\\
CTree & 0.995091 & 0.000066 & 0.005740 & 0.042931 & 8\\
\hline
\end{tabular}
\caption{Fidelity of K2204 linear baseline model and linear MBTs}
\label{tab:ins_k2204_lm_surrogates_perf}
\end{table}

GUIDE achieves the best performance slightly ahead of SLIM. CTree obtains the worst performance.
Since all algorithms generate MBTs with the same number of leaf nodes, the difference in performance must be explained by different split features or points.
Table \ref{tab:ins_k2204_lm_surrogates_share} lists the share of observations that were split with respect to the different features.

\begin{table}[!htb]

\centering \scriptsize
\begin{tabular}[t]{l|r|r|r}
\hline
& age & duration & sex\\
\hline
SLIM & 0.28 & 0.67 & 0.05\\
GUIDE & 0.28 & 0.72 & 0.00\\
MOB & 0.10 & 0.77 & 0.13\\
CTree & 0.00 & 0.96 & 0.04\\
\hline
\end{tabular}
\caption{Share of observations split by the different features K2204 linear MBTs}
\label{tab:ins_k2204_lm_surrogates_share}
\end{table}


It is noticeable that SLIM and GUIDE split by age more often than the other two algorithms.
Furthermore, it should be considered that particularly the SLIM tree could be influenced by selection bias and therefore sex with only one possible split point could be disadvantaged as a splitting variable. SLIM actually chooses sex less often as splitting variable than MOB and CTree, but sex is also rarely chosen by GUIDE and no selection bias in the independence case between numerical variables with different numbers of splitting variables could be found in GUIDE in chapter \ref{selection}. 
Moreover, the effect of selection bias would not be so dramatic here, since the two variables with which sex could interact - and probably does to a small extent, as the varying parameter estimates indicate - are chosen as splitting variables. The small interaction of sex with age and duration is thus reflected in the model, even if sex is not chosen as a splitting variable.

\subsubsection{MBTs with B-spline models}

In order to better capture nonlinearities and thus reduce the risk of splitting with respect to nonlinearities instead of interactions, all MBT algorithms are fitted with B-spline transformed feature age and duration as surrogate models. 
Two different maximal depths are used, 3 for interpretable shallow trees and 6 for deep trees with higher fidelity. The settings for $alpha$, $impr$ and minimum node size remain the same as for the MBTs with linear models.  Again, a baseline model is fitted, in this case a regression model with the feature sex and B-spline transformed features age and duration on the entire feature space. 

Figure \ref{fig:ins_k2204_fit} plots the prediction of the baseline B-spline model and the two B-spline SLIM surrogates against BPV\_pred to visualise performance improvement. This shows a considerable improvement from the baseline model to the shallow tree. For the deep tree, the observations seem to be even somewhat closer to the identity line. 

\begin{figure}[!htb]
    \centering    
    \includegraphics[width = 14cm]{figures/fit.png}
    \caption{B-spline surrogate predictions vs. BPV\_pred for K2204}
    \label{fig:ins_k2204_fit}
\end{figure}

The fidelity results for all B-spline surrogates are listed in Table \ref{tab:ins_k2204_bsplines_surrogates_perf} .

\begin{table}[!htb]
\centering \scriptsize
\begin{tabular}[t]{l|r|r|r|r|r}
\hline
  & $R^2$ & MSE & MAE & max AE & n leaves\\
\hline
B-spline baseline model & 0.9943311 & 7.63e-05 & 0.0067811 & 0.0378568 & 1\\
\hline
SLIM shallow & 0.9994176 & 7.80e-06 & 0.0018244 & 0.0167730 & 8\\
GUIDE shallow & 0.9993900 & 8.20e-06 & 0.0019011 & 0.0165545 & 8\\
MOB shallow & 0.9992115 & 1.06e-05 & 0.0022236 & 0.0182034 & 8\\
CTree shallow & 0.9990918 & 1.22e-05 & 0.0024194 & 0.0183906 & 8\\
\hline
SLIM deep & 0.9997514 & 3.30e-06 & 0.0010766 & 0.0126778 & 21\\
GUIDE deep & 0.9997301 & 3.60e-06 & 0.0011730 & 0.0116453 & 20\\
MOB deep & 0.9996858 & 4.20e-06 & 0.0013448 & 0.0119785 & 21\\
CTree deep & 0.9997091 & 3.90e-06 & 0.0012936 & 0.0123686 & 20\\
\hline
\end{tabular}
\caption{Fidelity of K2204 B-spline baseline model and  B-spline MBTs}
\label{tab:ins_k2204_bsplines_surrogates_perf}
\end{table}


The improvement of the shallow MBTs over the baseline model is large, but not as substantial as in the trees with linear models without B-spline transformations. This is probably due to the fact that the splits in the MBTs with linear models also handled nonlinearities that could not be adjusted in the linear baseline model. In the baseline model with B-spline transformations, on the other hand, the nonlinearities are already taken into account and the splits then actually capture primarily the interactions, which is what is desired. 
The deeper splitting improves the performance of all MBTs considerably. The MAE of the deep trees, for example, is only 52\%-61\% of the MAE of the shallow trees. CTree achieves the greatest improvement and obtains better fidelity in the deep trees than MOB (except for max AE). The better performance of all MBTs, however, comes at the cost of interpretability. Additionally, there is an increased risk of overfitting.




\begin{table}[!htb]
\centering \scriptsize
\begin{tabular}[t]{l|r|r|r}
\hline
  & age & duration & sex\\
\hline
SLIM shallow & 0.38 & 0.62 & 0.00\\
GUIDE shallow & 0.30 & 0.70 & 0.00\\
MOB shallow & 0.08 & 0.84 & 0.08\\
CTree shallow & 0.23 & 0.71 & 0.07\\
\hline
SLIM deep & 0.35 & 0.60 & 0.04\\
GUIDE deep & 0.20 & 0.78 & 0.02\\
MOB deep & 0.08 & 0.76 & 0.16\\
CTree deep & 0.20 & 0.67 & 0.13\\
\hline
\end{tabular}
\caption{Share of observations split by the different features K2204 B-spline MBTs}
\label{tab:ins_k2204_bsplines_surrogates_share}
\end{table}

Table \ref{tab:ins_k2204_bsplines_surrogates_share}  shows the proportions of observations that were split according to the different features. 
For SLIM, GUIDE and MOB the share results of the shallow trees are similar to the MBTs with linear models. Shallow CTree, on the other hand, selects age in $23\%$ of split observations as splitting variable, whereas it was not used at all for splitting in CTree with linear models. It performs the worst in terms of fidelity in this case as well, but not as considerable as in the previous setting.
With the deep trees, the values for share and also the fidelity values of the different MBTs move closer together.



For the interpretation, the shallow SLIM B-spline tree shown in Figure \ref{fig:ins_slim_bsplines_tree} is analysed in more detail.

\begin{figure}[!htb]
    \centering   
    \includegraphics[width = 16cm]{figures/slim_bsplines_small_tree.png}
    \caption{SLIM tree for K2204 with B-spline models}
    \label{fig:ins_slim_bsplines_tree}
\end{figure}

In order to investigate the effects of the splits on the feature effects more closely, the splits with regard to duration and age are analysed separately.
The nodes 1,5,13 and 14 together comprise the entire feature space, whereby the sub-regions are determined by splits with regard to the feature duration.
Figure \ref{fig:ins_k2204_effects_duration} shows the input-output relation (feature effects) of the features estimated in the B-spline models in the different nodes. Note that the curves are centred.

\begin{figure}[!htb]
    \centering
    \includegraphics[width = 16cm]{figures/effects_duration.png}
    \caption{Input-output relation of features in nodes split by duration for SLIM tree with B-splines and depth 3}
    \label{fig:ins_k2204_effects_duration}
\end{figure}

As with SLIM with linear models, it can be seen that the positive effect of sex male seems to increase with increasing duration. The same applies to age. The seemingly negative effect of age at low duration and high age is probably due to extrapolation, as there are only
few observations in this area, which is shown in Figure \ref{fig:app_ins_k2204_hist_age} in the appendix.



With the feature duration, it can be seen that the negative effect seems to decrease with increasing duration, which is again just a nonlinearity.

To investigate the effect of splits with respect to feature age, on the one hand nodes 4,7 and 8 are compared, which cover the feature space for duration $\leq 25$, and on the other hand nodes 11 and 12, which cover the feature space for $25 < $ duration $<= 40$. In the Figures \ref{fig:ins_k2204_effects_age_low_duration} and \ref{fig:ins_k2204_effects_age_medium_duration} the corresponding input-output relations of the features are shown.

\begin{figure}[!htb]
    \centering    
    \includegraphics[width = 16cm]{figures/effects_age_low_duration.png}
    \caption{Input-output relation of features in nodes with duration $\leq 25$ split by age for SLIM tree with B-splines and depth 3}
    \label{fig:ins_k2204_effects_age_low_duration}
\end{figure}

\begin{figure}[!htb]
    \centering    
    \includegraphics[width = 16cm]{figures/effects_age_medium_duration.png}
    \caption{Input-output relation of features in nodes with $25 < $ duration $<= 40$ split by age for SLIM tree with B-splines and depth 3}
    \label{fig:ins_k2204_effects_age_medium_duration}
\end{figure}

Again, the interpretation is consistent with the results from SLIM with linear models. The positive effect of sex and age is increased by increasing age, while the negative effect of duration is reduced. The slightly negative effect of age at high age and low duration should again be viewed with caution and is probably due to the poor data situation in this area.


Finally, a deep SLIM tree with B-spline models is used as a standalone model for BPV and its accuracy is compared to the accuracy of the black box model. The result is shown in Table \ref{tab:ins_k2204_standalone_slim}.
The accuracy of SLIM is worse than that of the black box model for all evaluation measures. However, the difference is most apparent for the max AE. While the max AE is explicitly minimised in the black box model, the MSE is minimised with SLIM. In general, a different loss function would also be possible with SLIM. In this case, either the max AE could be minimised only in the split selection, or also in the modelling in the nodes. When optimising the max AE in the split selection, it must be noted that the algorithm is principally designed for additive loss functions. In order to compare the joint performance of the child models with that of the parent model, the maximum should probably be used instead. 
However, it is questionable whether the data would be split according to interactions in this case, especially if the models were nevertheless fitted using least squared regression.

\begin{table}[!htb]

\centering \scriptsize
\begin{tabular}[t]{l|r|r|r|r}
\hline
  & $R^2$ & MSE & MAE & max AE \\
\hline
SLIM & 0.9997757 & 3.1e-06 & 0.0010172 & 0.0118951\\
Blackbox model & 0.9998316 & 2.3e-06 & 0.0009441 & 0.0047668\\
\hline
\end{tabular}
\caption{Accuracy of standalone B-spline SLIM MBTs and of the black box model K2204}
\label{tab:ins_k2204_standalone_slim}
\end{table}








\subsection{Data set R1\_08}

The data set R1\_08 contains the data of an annuity insurance tariff. Instead of a single benefit in the endowment case, a lifelong annuity is paid out.
R1\_08 includes, in addition to sex, age and duration, the features birth\_year, payment\_period, in\_year\_payments\_exkasso (categorical with 4 levels), guarantee\_period and increment\_factor.
The value range of the features age and duration is limited to a range in which no correlation exists ($25 \leq$ age $\leq 35$ and $30 \leq$ duration $\leq 40$).
 Here, as well, the BPV and BPV\_pred predicted by a black box model are analysed as target variables.
For the application of the MBTs, subsets of the training and test data sets including BPV and BPV\_pred are drawn, each with 100000 observations.

In order to model nonlinearities in the nodes, MBTs with B-spline models are used. As with K2204, trees with two different depths are evaluated, shallow trees with a maximum depth of 3 and deep trees with a maximum depth of 7. $impr$ and $alpha$ are set to 0.05 and a minimum node size of 500 observations is required.

For the interpretation of the splits and models, the shallow SLIM tree is examined in more detail. Its structure is shown in Figure \ref{fig:ins_k108_slim_bsplines_small_tree}.
If the tree is fitted on the test data instead of the training data, exactly the same splits result. The same applies if the tree is used as a standalone model for BPV instead of a surrogate model. This indicates that the black box model replicates the true data and relationships well.


\begin{figure}[!htb]
    \centering
    \includegraphics[width = 16cm]{figures/slim_bsplines_small_tree.png}
    \caption{Shallow SLIM tree for K1\_08 with B-spline models}
    \label{fig:ins_k108_slim_bsplines_small_tree}
\end{figure}


It is noticeable that the feature space in the first splits is only divided with regard to increment\_factor. The effects of these splits on the other features are shown in Figure \ref{fig:ins_k108_effects_increment}.

\begin{figure}[!htb]
    \centering    
    \includegraphics[width=16cm]{figures/effects_increment_factor.png}
    \caption{Input-output relation of features in nodes split by increment\_factor for SLIM tree with B-splines and depth 3}
    \label{fig:ins_k108_effects_increment}
\end{figure}

The effects of the features payment\_period and guarantee\_period are not shown because they are very small and therefore not visible on the scale at all.
The interaction with increment\_factor is clearly visible in all the features shown. For all features, an increasing increment\_factor increases the feature effects.


The consequences of the splits with respect to duration are shown in Figure \ref{fig:ins_k108_effects_duration}. It indicates that across all features a higher duration weakens the feature main effects.

\begin{figure}[!htb]
    \centering 
    \includegraphics[width=16cm]{figures/effects_duration.png}
    \caption{Input-output relation of features in nodes split by duration for SLIM tree with B-splines and depth 3 (nodes 11-14)}
    \label{fig:ins_k108_effects_duration}
\end{figure}


Since increment\_factor interacts with so many features, the splits are very effective here and bring a great improvement in performance. Table \ref{tab:ins_k108_share} lists the share of the splits by the different features. From this it can be seen that MOB and CTree split shallow MBTs considerably less by increment\_factor than SLIM and GUIDE. At the same time, their performance is behind that of SLIM and GUIDE, as can be seen in Table \ref{tab:ins_k108_bsplines_surrogates_perf}. SLIM achieves the best performance.






By using deep trees, the fidelity increases and the results of the different algorithms move closer together. The values for share also get closer. Overall, the differences between the different algorithms are therefore less pronounced with the deep trees than with the shallow trees. Although the deep trees achieve a high training performance, an interpretation is hardly possible with this high number of leaf nodes. In addition, the test performance differs more strongly from the training performance than with the shallow trees, which is a sign of overfitting. The almost identical values for max AE have been checked and are correct. They result from the same observation for all four algorithms and the observation falls in nodes with almost identical subregions. This shows again that the MTBs or, more precisely, the subregions found by the different algorithms and thus also their performance move closer together when deep MBTs are formed.

\begin{table}[!htb]

\centering \tiny
\begin{tabular}[t]{l|r|r|r|r|r|r|r|r|r}
\hline
& \multicolumn{4}{|c|}{train} & \multicolumn{4}{|c|}{test} & \\
\hline
 & $R^2$ & MSE & MAE & max AE & $R^2$ & MSE & MAE & max AE & n leaves\\
\hline

B-spline & 0.927748 & 3.534102 & 1.291762 & 16.412655 & 0.927267 & 3.558816 & 1.295778 & 16.413200 & 1\\
\hline
SLIM shallow & 0.997432 & 0.125606 & 0.235344 & 4.296943 & 0.997397 & 0.127386 & 0.236761 & 4.299219 & 8\\
GUIDE shallow & 0.996540 & 0.169233 & 0.262321 & 5.006522 & 0.996496 & 0.171433 & 0.263770 & 5.003334 & 8\\
MOB shallow & 0.994944 & 0.247289 & 0.324474 & 5.236252 & 0.994942 & 0.247489 & 0.324895 & 5.336406 & 8\\
CTree shallow & 0.993049 & 0.340023 & 0.401982 & 5.236252 & 0.993055 & 0.339838 & 0.401632 & 5.336406 & 8\\
\hline
SLIM deep & 0.999882 & 0.005794 & 0.043939 & 1.079069 & 0.999870 & 0.006350 & 0.045885 & 1.126732 & 105\\
GUIDE deep & 0.999844 & 0.007652 & 0.052102 & 1.079069 & 0.999832 & 0.008219 & 0.054046 & 1.126732 & 95\\
MOB deep & 0.999861 & 0.006823 & 0.047428 & 1.079069 & 0.999848 & 0.007460 & 0.049459 & 1.126732 & 108\\
CTree deep & 0.999839 & 0.007851 & 0.058806 & 1.079069 & 0.999825 & 0.008539 & 0.061363 & 1.126732 & 106\\
\hline
\end{tabular}
\caption{fidelity of K1\_08 B-spline baseline model and  B-spline MBTs K2204}
\label{tab:ins_k108_bsplines_surrogates_perf}
\end{table}




\begin{table}[!htb]
\centering \scriptsize
\begin{tabular}[t]{l|r|r|r|r|r}
\hline
  & sex & age & duration & birth\_year & increment\\
\hline
SLIM shallow & 0.00 & 0.00 & 0.12 & 0.00  & 0.88\\
GUIDE shallow & 0.00 & 0.12 & 0.00 & 0.00  & 0.88\\
MOB shallow & 0.00 & 0.12 & 0.33 & 0.00  & 0.54\\
CTree shallow & 0.00 & 0.33 & 0.33 & 0.00  & 0.33\\
\hline
SLIM deep & 0.10 & 0.08 & 0.24 & 0.05 & 0.54\\
GUIDE deep & 0.06 & 0.10 & 0.22 & 0.05 & 0.56\\
MOB deep & 0.11 & 0.15 & 0.20 & 0.03 & 0.52\\
CTree deep & 0.00 & 0.17 & 0.29 & 0.05 & 0.49\\
\hline
\end{tabular}
\caption{Share of observations split by the different features K1\_08 B-spline MBTs}
\label{tab:ins_k108_share}
\end{table}

The feature payment\_period, in\_year\_payments\_exkasso and guarantee\_period are never chosen as splitting variables and are therefore not listed in the table.


Finally two SLIM trees with B-spline models are fitted as  standalone models for BPV and their accuracy is compared with the black box model. The result is shown in Table \ref{tab:ins_k108_standalone_slim}. For this data set, too, the deviations are most considerable for the max AE





\begin{table}[!htb]

\centering \scriptsize  
\begin{tabular}[t]{l|r|r|r|r|r|r|r|r}
\hline
 & \multicolumn{4}{|c|}{train} & \multicolumn{4}{|c}{test} \\
\hline
 & $R^2$ & MSE & MAE & max AE & $R^2$ & MSE & MAE & max AE \\
\hline
SLIM shallow & 0.9974321 & 0.1256075 & 0.2353447 & 4.3046812 & 0.9973966 & 0.1273854 & 0.2367417 & 4.3074899\\
SLIM deep & 0.9998814 & 0.0057987 & 0.0439357 & 1.0862638 & 0.9998702 & 0.0063532 & 0.0458758 & 1.1344576\\
Blackbox & 1.0000000 & 0.0000023 & 0.0011006 & 0.0096827 & 1.0000000 & 0.0000023 & 0.0010968 & 0.0099144\\
\hline
\end{tabular}
\caption{Accuracy of standalone B-spline SLIM MBTs and of the black box model K1\_08}
\label{tab:ins_k108_standalone_slim}
\end{table}

The results of the application of the MBT algorithms were discussed with an expert and the plausibility of the resulting interpretations was verified.

==> chapters/main-labels.tex <==

\newlabel{intro}{{1}{1}{Introduction}{section.1.1}{}}
\newlabel{related}{{2}{3}{Related Work}{section.1.2}{}}
\newlabel{background}{{3}{4}{Background: Model-Based Trees}{section.1.3}{}}
\newlabel{tab:mbt_comparison}{{1}{5}{Comparison of MBT algorithms}{table.1.1}{}}
\newlabel{simulation}{{4}{7}{Comparison Study}{section.1.4}{}}
\newlabel{sec:experiments}{{4.2}{8}{Experiments}{subsection.1.4.2}{}}
\newlabel{tab:simulation_setting}{{2}{9}{Definition of variants for all simulation settings}{table.1.2}{}}
\newlabel{sec:lin_smooth}{{4.2}{9}{Linear smooth}{section*.15}{}}
\newlabel{tab:linear_smooth_summary}{{3}{10}{Simulation results on 100 simulation runs for all four MBTs as surrogate models on the scenario linear smooth with sample sizes $n_{train}=1000$ and $n_{test} = 500$ for different values of $\gamma $ and $\alpha $. The mean (standard deviation) fidelity on the training data for the lm is 0.9902 (0.0006) and for the XGBoost is 0.9858 (0.0008). On the test data set the respective fidelity values for the lm are 0.9901 (0.0008) and for the XGBoost are 0.9768 (0.0018)}{table.1.3}{}}
\newlabel{fig:ls_1000_xgboost_r2_train}{{1}{11}{RI for the four MBT algorithms when used as surrogate model for an XGBoost model for the scenario linear smooth with $n_{train}=1000$ and $n_{test} = 500$, $\alpha = \gamma = 0.05$. The numbers below the boxplots indicate the number of tree pairs, for which both trees have the respective number of leaf nodes}{figure.1.1}{}}
\newlabel{fig:la_1000_standalone_r2_test}{{2}{12}{Test accuracy $R^2$ vs. number of leaf nodes for the four MBT algorithms as surrogate models for XGBoost for scenario linear categorical with $n_{train}=1000$ and $n_{test} = 500$, $\alpha = \gamma = 0.05$. The numbers below the boxplots indicate the number of trees (from 100 simulation runs) which have the respective number of leaf nodes for the regarded algorithm}{figure.1.2}{}}
\newlabel{fig:lm_1000_standalone_r2_test}{{3}{13}{Test accuracy $R^2$ vs. number of leaf nodes for the four MBT algorithms when used as surrogate model on the xgboost model for scenario linear mixed with $n_{train}=1000$ and $n_{test} = 500$, $\alpha = \gamma = 0.05$. The numbers below the boxplots indicate the number of trees (from 100 simulation runs) which have the respective number of leaf nodes for the regarded algorithm}{figure.1.3}{}}
\newlabel{fig:lm_1000_standalone_share_x3x4}{{4}{14}{Relative amount of partitions which use features $\textbf {x}_3, \textbf {x}_4$ for splittings vs. the number of leaf nodes for the four MBT algorithms when the XGBoost model is used as surrogate model for the scenario linear mixed with $n=1500, \alpha = \gamma = 0.05$}{figure.1.4}{}}
\newlabel{fig:lm_1000_standalone_lm_sta}{{5}{14}{RI for the four MBT algorithms when used as surrogate model for the scenario linear mixed with $n_{train}=1000$ and $n_{test} = 500$, $\alpha = \gamma = 0.05$. The numbers below the boxplots indicate the number of tree pairs (from 4950 pairs), for which both trees have the respective number of leaf nodes}{figure.1.5}{}}
\newlabel{conclusion}{{5}{15}{Discussion}{section.1.5}{}}

